Fast Robust Methods for Singular State-Space Models

State-space models are used in a wide range of time series analysis formulations. Kalman filtering and smoothing are work-horse algorithms in these settings. While classic algorithms assume Gaussian errors to simplify estimation, recent advances use a broader range of optimization formulations to allow outlier-robust estimation, as well as constraints to capture prior information. Here we develop methods on state-space models where either innovations or error covariances may be singular. These models frequently arise in navigation (e.g. for `colored noise' models or deterministic integrals) and are ubiquitous in auto-correlated time series models such as ARMA. We reformulate all state-space models (singular as well as nonsinguar) as constrained convex optimization problems, and develop an efficient algorithm for this reformulation. The convergence rate is {\it locally linear}, with constants that do not depend on the conditioning of the problem. Numerical comparisons show that the new approach outperforms competing approaches for {\it nonsingular} models, including state of the art interior point (IP) methods. IP methods converge at superlinear rates; we expect them to dominate. However, the steep rate of the proposed approach (independent of problem conditioning) combined with cheap iterations wins against IP in a run-time comparison. We therefore suggest that the proposed approach be the {\it default choice} for estimating state space models outside of the Gaussian context, regardless of whether the error covariances are singular or not.

==> optimization.tex <==
\section{Efficient Splitting Methods for Singular Kalman Smoothing}
\label{sec:Opt}


We consider problems of the form

\begin{equation}
\min_{z} \rho(z) \quad \mbox{s.t.} \quad Az = \hat w. 
\label{eq:main}
\end{equation}

Where
\[
\rho(z) = \rho_1(u) + \rho_2(t) + \rho_3(x),
\]
With $\rho_1, \rho_2, \rho_3$ al PLQ (piecewise linear quadratic) functions.


\subsection{Overall optimization: DRS}

To solve (\ref{eq:main}) we employ a Douglas-Rachford splitting algorithm. This is an iterative primal-dual algorithm with each iteration consisting of two sub-problems:

\begin{equation}
\lambda^{n+1} = \prox_{\sigma \rho^*}(\lambda^n + \sigma \bar{z}^n) = \argmin_x \frac{1}{2\sigma}\|x-\lambda^n - \sigma \bar{z}^n\|^2 + \rho*(\lambda^n + \sigma \bar{z}^n )
\label{eq:proxsub}
\end{equation}

\begin{equation}
z^{n+1} = \arg\min_t \|t - z^n + \tau \lambda^{n+1}\|^2 \quad \text{ s.t. } At = \hat{w}
\label{eq:lssub}
\end{equation}

And a momentum term:

\[
\bar{z}^{n+1} = 2z^{n+1} - z^n
\]

For problems of type (\ref{eq:main}) the DRS algorithm converges locally linearly to a solution. This can be shown by replicating an argument in \cite{LFP} which uses metric subregularity of operators to show linear convergence.  We recall the definition of metric subregulairty:

\begin{definition} A mapping $F: \mathbb{R}^n \rightrightarrows \mathbb{R}^m$ is called \textit{metrically subregular} at $\bar{x}$ for $\bar{y}$ if $(\bar{x}, \bar{y}) \in $ gra $F$ and there exists $\eta \in [0 , infty)$, neighborhoods $\mathcal{U}$ of $\bar{x}$, and $\mathcal{Y}$ of $\bar{y}$ such that 
\[
d(x, F^{-1}\bar{y}) \leq \eta d(\bar{y}, Fx \cap \mathcal{Y}), \quad \forall x \in \mathcal{U}
\]
\end{definition}

In \cite{LFP} they argue that all PLQ functions have subdifferentials that are metrically subregular. To apply their argument to the case of (\ref{eq:main}) we additionally need to verify that the subdifferential of the indicator function for a affine subspace is also metrically subregular. However this follows from the quadratic growth condition for subdifferentials of convex functions , namely 

\begin{theorem}[\cite{AG}, Theorem 3.3]
For a proper closed convex function $f$, the subdifferential $\partial f$ is metrically subregular at $\bar{x}$ for $\bar{y}$ with $(\bar{x}, \bar{y}) \in $ gra $\partial f$ if and only if there exists a positive constant $c$ and a neighborhood $\mathcal{U}$ of $\bar{x}$ such that

\[
f(x) \geq f(\bar{x}) + \langle \bar{y}, x-\bar{x}\rangle + cd^2(x, (\partial f)^{-1}(\bar{y})), \quad \forall x \in \mathcal{U}
\]

\end{theorem}

In the case that $f$ is an indicator function there is nothing to check, it is true by definition of $\partial f$. Now the same proof as in \cite{LFP} will show local linear convergence.
With a fast convergence rate established we now turn to per-iteration complexity as the best way to increase performance.
\subsection{Proximity operators for $\rho$}

We define 
\[
\prox_{\gamma \rho}(z) = \arg\min_x \frac{1}{2\gamma}\|x-z\|^2 + \rho(x).
\]

The proximity operator appearing in the sub-problem of DRS involves $\rho^*$ instead of $\rho$ so we apply the Moreau decomposition to relate the proximity operator of $\rho$ and $\rho^*$ by

\[
\prox_{\sigma \rho}(z) + \sigma \prox_{\rho^*/\sigma}(z/\sigma) = z
\]

Thus only $\prox_{\rho}(z)$ needs to be computed. By assumption $\rho(z) = \rho_1(u) + \rho_2(t) + \rho_3(x)$ thus computing $\prox_{\rho}(z)$ reduces to separately computing $\prox_{\rho_1}(u)$, $\prox_{\rho_2}(t)$, $\prox_{\rho_3}(x)$. For complexity analysis of DRS we assume that all of these proximal functions can be computed via an algorithm that converges linearly.

This assumption is automatically satisfied if $\rho_i, i=1,2,3$ are PLQ (piecewise linear quadratic) by using an interior point method. This assures that our assumption is not very restrictive as the class of PLQ functions is quite large and includes many common choices of penalty functions such as $\|\cdot\|_1, \|\cdot\|_2^2$, the huber loss function, and many others. A number of PLQ functions and their computed proximal operators are discussed in the appendix. 



\subsection{Proximity operator for constraint}

In each iteration (\ref{eq:lssub}) takes the form:

\[
\min_{At = w} \frac{1}{2}\|t - c\|^2. 
\]

Where $c$ is a constant that changes from iteration to iteration. Examining optimality conditions we see that finding the optimum is equivalent to solving the linear system
\[
\begin{bmatrix}I & A^T\\A & 0\end{bmatrix}\begin{bmatrix}t\\ \nu\end{bmatrix} = \begin{bmatrix}c\\ \hat{w}\end{bmatrix}
\]

Which can be written equivalently 

\[
\begin{bmatrix}I & A^T\\0 & AA^T\end{bmatrix} \begin{bmatrix}t\\ \nu\end{bmatrix} = \begin{bmatrix}c\\ Ac - \hat{w}\end{bmatrix}
\]

Thus solving $AA^T \nu = Ac - \hat{w}$ then back substitution will yield the optimal $t$. As $AA^T$ appears in every iteration we compute a  factorization of this matrix once before implementing the algorithm and use this to efficiently solve (\ref{eq:lssub}) in every iteration.

\subsection{Factorization of $AA^T$}

Recall from the definition that $A$ is lower block bi-diagonal and thus $AA^T$ is block tri-diagonal. We will compute the Cholesky factorization of $AA^T = LL^T$ Where $L$ is a square block bi-diagonal matrix. This can be done efficiently by iterating through the blocks of $AA^T$ as follows. Let

\[
AA^T = 
\begin{bmatrix}
a_1& b_1^T & & \\
b_1 & a_2 & b_2^T & \\
& b_2 & a_3 & b_3^T \\
&&b_3 & a_4
\end{bmatrix}
\quad 
L = 
\begin{bmatrix}
c_1& & & \\
d_1 & c_2 &  & \\
& d_2 & c_3 &  \\
&&d_3 & c_4
\end{bmatrix}
\]

Multiplying out $LL^T$ it follows that

\[
a_1 = c_1c_1^T, \quad d_1 = b_1 c_1^{-T}
\]

Thus to compute $c_1$ we simple compute the Cholekly factorization of $a_1$. Then

\[
c_2c_2^T = a_2 - b_1a_1^{-1}b_1^T, \quad d_2 = b_2c_2^{-1}. 
\]

Take $s_1 = a_1$, and proceeding recursively, we have 

\[
s_k = a_k - b_{k-1}s_{k-1}^{-1}b_{k-1}^T
\]

and 

\[
c_kc_k^T = s_k, \quad d_k = b_kc_k^{-1}.
\]

$c_k$ is then found by finding the Cholesky factorization of $s_k$, then $c_k$ is inverted to find $d_k$.
The overall speed of computing this factorization is not of great importance as it only will be computed a single time.
Once $L$ has been computed we can solve $LL^T \nu = Ac - \hat{w}$ in $O(n^2N)$ operations as the blocks of $L$ are triangular.


==> vehicleModel.tex <==
\section{Vehicle Model}
\label{sec:vehicleModel}

The filter fuses depth, gyrocompass, and linear acceleration data from
the vehicle. A description of the full nonlinear process model is
presented in Section \ref{sec:nonlin_pm}, the linear simplification in
Section \ref{sec:lin_pm}, the process prodiction in in Section
\ref{sec:proc_pred}, and the measurement models in Section
\ref{sec:meas_model}.

\subsection{Nonlinear Process Model}
\label{sec:nonlin_pm}
The complete state vector, denoted $\vect{x}$, contains pose and attitude, as
well as body-frame linear and angular velocities
%
\begin{equation}
  \vect{x} = [\vect{s}^\top,\vect{\varphi}^\top,\vect{\upsilon}^\top,\vect{\omega}^\top]^\top
\end{equation}
\begin{equation}
  \vect{s} = \left[\begin{array}{c}
      x \\
      y \\
      z \end{array}\right],~
  \vect{\varphi} = \left[\begin{array}{c}
      r \\
      p \\
      h \end{array}\right],~
  \vect{\upsilon} = \left[\begin{array}{c}
      u \\
      v \\
      w \end{array}\right],~
  \vect{\omega} = \left[\begin{array}{c}
      a \\
      b \\
      c \end{array}\right]
\end{equation}
%
where $\vect{s}$ is the vehicle pose in the local frame,
$\vect{\varphi}$ is the vehicle attitude (Euler roll,
pitch, heading), $\vect{\upsilon}$ is the body-frame linear velocity,
and $\vect{\omega}$ is the body-frame angular velocity.

The filter uses a vehicle-agnostic constant-velocity process model for the
vehicle, which is defined as
%
\begin{align}
\dot{\vect{x}} &= 
\underbrace{\left[\begin{array}{cccc}
\mtrx{0}&\mtrx{0}&\mtrx{R}(\vect{\varphi})&\mtrx{0} \\
\mtrx{0}&\mtrx{0}&\mtrx{0}&\mtrx{\mathcal{J}(\vect{\varphi})} \\
\mtrx{0}&\mtrx{0}&\mtrx{0}&\mtrx{0} \\
\mtrx{0}&\mtrx{0}&\mtrx{0}&\mtrx{0} \end{array}\right] \vect{x}}_{\mbox{$\vect{f}(\vect{x}(t))$}} + 
\underbrace{\left[\begin{array}{cc}
\mtrx{0}&\mtrx{0} \\
\mtrx{0}&\mtrx{0} \\
\mtrx{I}&\mtrx{0} \\
\mtrx{0}&\mtrx{I} \end{array}\right]}_{\mbox{$\mtrx{G}$}} \vect{w} \label{x_v-dot}
\end{align}
%
where $\mtrx{R}(\vect{\varphi})$ is the transformation from body-frame
to local-level linear velocities, $\mtrx{\mathcal{J}}(\vect{\varphi})$
is the transformation from body-frame angular velocities to Euler
rates, and $\vect{w} \sim \mathcal{N}(0,\mtrx{Q})$ is zero-mean
Gaussian process noise in the velocity
term. $\mtrx{R}(\vect{\varphi})$ and
$\mtrx{\mathcal{J}}(\vect{\varphi})$ are found by solving
%
\begin{equation}
  \mtrx{R}(\vect{\varphi}) = \mtrx{R}^\top_h \mtrx{R}^\top_p \mtrx{R}^\top_r
\end{equation}
where
\begin{equation}
  \mtrx{R}_{h} = \left[\begin{array}{ccc}
      \cos{h} & \sin{h} & 0 \\
      -\sin{h} & \cos{h} & 0 \\
      0 & 0 & 1 \end{array}\right], ~% \nonumber\\
%
  \mtrx{R}_{p} = \left[\begin{array}{ccc}
      \cos{p} & 0 & -\sin{p} \\
      0 & 1 & 0 \\
      \sin{p} & 0 & \cos{p} \end{array}\right], ~ %\nonumber\\
%
  \mtrx{R}_{r} = \left[\begin{array}{ccc}
      1 & 0 & 0 \\
      0 &\cos{r} & \sin{r} \\
      0 & -\sin{r} & \cos{r} \end{array}\right] %\nonumber
\end{equation}
and
\begin{align}
  \vect{\omega} &= \left[\begin{array}{c} \dot{r} \\ 0 \\
      0 \end{array}\right] + R_r \left[\begin{array}{c} 0 \\
      \dot{p} \\ 0 \end{array}\right] + R_r R_p
  \left[\begin{array}{c}
      0 \\ 0 \\ \dot{h} \end{array}\right] \nonumber\\
 &= \underbrace{\left[\begin{array}{ccc}
      1 & 0 & -\sin{p} \\
      0 & \cos{r} & \sin{r} \cos{p} \\
      0 & -\sin{r} & \cos{r} \cos{p} \end{array}\right]
    }_{\mbox{$\mtrx{\mathcal{J}}^{-1}$}} \dot{\varphi}
\end{align}

\begin{align}
  \mtrx{\mathcal{J}} %&= \left[\begin{array}{ccc}
%      1 & 0 & -\sin{p} \\
%      0 & \cos{r} & \sin{r} \cos{p} \\
%      0 & -\sin{r} & \cos{r} \cos{p} \end{array}\right]^{-1} \nonumber\\
   &= \left[\begin{array}{ccc}
      1 & \sin{r}\tan{p} & \cos{r}\tan{p} \\
      0 & \cos{r} & -\sin{r} \\
      0 & \sin{r}\sec{p} & \cos{r} \sec{p} \end{array}\right] .
\end{align}
%
Note that the vehicle process model does not include a control input term
$\vect{u}(t)$ because we do not assume a dynamic model for the vehicle. The use
of a simple kinematic model makes the algorithm trivially applicable to any
vehicle, and is appropriate for many underwater vehicle applications because
accelerations are heavily damped by the water and autonomous vehicle's often are
used for survey work, which involves travelling in long straight lines.

We linearize the vehicle process model \eqref{x_v-dot} about
$\vect{\mu}$, our estimate of the vehicle state at time $t$, using
the Taylor series expansion
%
\begin{equation}\begin{split}
  \dot{\vect{x}}(t) &= \vect{f}(\vect{\mu}) +
  \mtrx{F}(\vect{x}(t) - \vect{\mu})\\
  &\quad+ HOT + \mtrx{G} \vect{w}(t)
\end{split}\end{equation}
%
where
\begin{equation}
\mtrx{F} = \left. \dfrac{\partial \vect{f}(\vect{x})}{\partial
  \vect{x}}\right|_{\vect{x}(t) = \vect{x}(t_k)}
\end{equation}
%
and $HOT $ denotes higher order terms. Dropping the $HOT$ and rearranging we get
\begin{align}
  \dot{\vect{x}}(t) &\approx \mtrx{F} \vect{x}(t) + \underbrace{\vect{f}(\vect{\mu}) - \mtrx{F} \vect{\mu}}_{\mbox{$\vect{u}(t)$}} + \mtrx{G} \vect{w}(t) \\
&= \mtrx{F} \vect{x}(t) + \vect{u}(t) + \mtrx{G} \vect{w}(t)  \label{linz}
\end{align}
where $\vect{f}(\vect{\mu}) - \mtrx{F} \vect{\mu}$ 
is treated as a constant pseudo-input term $\vect{u}(t) $. 


In order to discretize the linearized vehicle process model
we rewrite \eqref{linz} as
\begin{equation}
  \dot{\vect{x}}(t) = \mtrx{F} \vect{x}(t) + \mtrx{B} \vect{u}(t) + \mtrx{G} \vect{w}(t)
\end{equation}
%
where $\mtrx{B} = \mtrx{I}$.
%
Assuming zero-order hold and using the standard method
 \cite{ybarshalom-2001a} to discretize over a
time step $T$ we solve for $\mtrx{F}_{v_k}$ and $\mtrx{B}_{v_k}$ in
the discrete form of the process model:
%
\begin{align}
% this version has explicit t_k etc
%\vect{x}[t_{k+1}] &= \mtrx{F}_{v_k} \vect{x}[t_k] + \mtrx{B}_{v_k} \vect{u}[t_k] + \vect{w}[t_k] \label{disc_v}\\
% this version just has k and k-1 subscripts
\vect{x}_{v_{k+1}} &= \mtrx{F}_{v_k} \vect{x}_{v_k} + \mtrx{B}_{v_k} \vect{u}_k + \vect{w}_{v_k} \label{disc_v}\\
%
\mtrx{F}_{v_k} &= e^{\mtrx{F} T} \\
%
\mtrx{B}_{v_k} &= \int^T_0 e^{\mtrx{F} (T-\tau)}\mtrx{B} d\tau  \nonumber\\
&= e^{\mtrx{F} T}\int^T_0 e^{-\mtrx{F} \tau}d\tau.
\end{align}
%
The discretized process noise $\vect{w}_{v_k}$ has the form
\begin{equation}
\vect{w}_{v_k} = \int^T_0 e^{\mtrx{F} (T-\tau)}\mtrx{G} \vect{w}(\tau) d\tau
\end{equation}
%
for which we can calculate the mean: % and variance
\begin{align}
  E\left[\vect{w}_{v_k}\right] &=  E\left[ \int^T_0 e^{\mtrx{F} (T-\tau)}\mtrx{G} \vect{w}(\tau) d\tau \right] \label{mean}\\
  &= \int^T_0 e^{\mtrx{F} (T-\tau)}\mtrx{G} \cancelto{0}{E[\vect{w}(\tau)]} d\tau \nonumber\\
  &= 0. \nonumber
\end{align}

To calculate the variance of the discretized vehicle process noise we
make use of the facts that the expected value can be brought inside
the integral because it is a linear operator and that the noise vector
$\vect{w}$ is independent and identically distributed in time so that
the covariance $E\left[\vect{w}(\tau) \vect{w}^\top_v(\gamma)\right]$
is zero except when $\gamma = \tau$:
\begin{align}
\mtrx{Q}_{v_k} &= E\left[\vect{w}_{v_k}\vect{w}_{v_k}^\top\right]  \label{var}\\
 &= E\left[\int^T_0 e^{\mtrx{F} (T-\tau)}\mtrx{G} \vect{w}(\tau) d\tau \int^T_0 \left(e^{\mtrx{F} (T-\gamma)}\mtrx{G} \vect{w}(\gamma) \right)^\top d\gamma \right] \nonumber\\
 &= E\left[\int^T_0 \int^T_0 e^{\mtrx{F} (T-\tau)} \mtrx{G} \vect{w}(\tau) \vect{w}^\top_v(\gamma) \mtrx{G}^\top e^{\mtrx{F}^\top (T-\gamma)} d\tau d\gamma\right] \nonumber\\
 &= \int^T_0 \int^T_0 e^{\mtrx{F} (T-\tau)} \mtrx{G} \underbrace{E\left[\vect{w}(\tau) \vect{w}^\top_v(\gamma)\right]}_{\mbox{$\mtrx{Q} \delta(\tau-\gamma)$}} \mtrx{G}^\top e^{\mtrx{F}^\top (T-\gamma)}  d\tau d\gamma \nonumber\\
 &= \int^T_0 e^{\mtrx{F} (T-\tau)} \mtrx{G} \mtrx{Q} \mtrx{G}^\top e^{\mtrx{F}^\top (T-\tau)} d\tau. \nonumber
\end{align}


\subsection{Linear Process Model}
\label{sec:lin_pm}

For a vehicle that is well-instrumented in attitude, the uncertainty in position
(and the x-y states in particular) is typically orders of magnitude larger than
the uncertainty attitude. As such, in practice, we can often simplify the full
nonlinear vehicle process model to track only position, $\vect{s} =
\left[\begin{array}{ccc} x & y & z\end{array}\right]^\top$, while assuming that
the attitude, $\vect{\varphi} = \left[\begin{array}{ccc} r & p &
    h\end{array}\right]^\top$, can be known from the most recent sensor
measurements. To make the model linear, the position and its derivatives will all be
referenced to the local-level frame.
%
In addition, in order to incorporate linear accleration measurements from
an inertial measurement unit (IMU), we will include linear acceleration in
the state vector in addition to the linear velocities.  This leads to the state
vector
%
\begin{equation}
  \vect{x}_s = [x,y,z,\dot{x},\dot{y},\dot{z},\ddot{x},\ddot{y},\ddot{z}]^\top.
\end{equation} \label{lin_pm}
%

We still employ a linear constant-velocity process model, which simplifies to
%
\begin{align}
\dot{\vect{x}}_s &= 
\underbrace{\left[\begin{array}{ccc}
\mtrx{0} & \mtrx{I} & \mtrx{0} \\
\mtrx{0} & \mtrx{0} & \mtrx{I} \\
\mtrx{0} & \mtrx{0} & \mtrx{0} \end{array}\right]}_{\mbox{$\mtrx{F}_s$}} \vect{x}_s + 
\underbrace{\left[\begin{array}{c}
\mtrx{0} \\
\mtrx{I} \\
\mtrx{0} \end{array}\right]}_{\mbox{$\mtrx{G}_s$}} \vect{w}_s \label{x_s-dot},
\end{align}
%
where $\vect{w}_s \sim \mathcal{N}(0,\mtrx{Q}_s)$ is zero-mean
Gaussian process noise, which we still inlcude in the veloity term.

The linear process model \eqref{x_s-dot} is
discretized in the same fashion as the nonlinear vehicle process model:
%
\begin{align}
% this version has explicit t_k etc
%\vect{x}_s[t_{k+1}] &= \mtrx{F}_{s_k} \vect{x}_s[t_k] + \vect{w}_s[t_k] \label{disc_s}\\
% this version uses k and k-1 subscripts
\vect{x}_{s_{k+1}} &= \mtrx{F}_{s_k} \vect{x}_{s_k} + \vect{w}_{s_k} \label{disc_s}\\
\mtrx{F}_{s_k} &= e^{\mtrx{F}_s T}\\
 &= \mtrx{I} + \mtrx{F}_sT + \cancelto{0}{\frac{1}{2!}\mtrx{F}_s^2T^2} + \cancelto{0}{\frac{1}{3!}\mtrx{F}_s^3T^3} + \cdots \nonumber\\
 &= \left[\begin{array}{ccc}
\mtrx{I}&\mtrx{I}T&\mtrx{0}\\
\mtrx{0}&\mtrx{I}&\mtrx{I}T\\
\mtrx{0}&\mtrx{0}&\mtrx{I} \end{array} \right] \nonumber
\end{align}
where the higher order terms are {\it identically zero} because of the
structure of $\mtrx{F}_s$, resulting in a simple closed-form solution
for $\mtrx{F}_{s_k}$. Note that $\mtrx{B}_{s_k} = \mtrx{0}$ because
$\mtrx{B}_s = \mtrx{0}$.
%
The discretized process noise
\begin{equation}
  \vect{w}_{s_k} = \int^T_0 e^{\mtrx{F}_s(T - \tau)}\mtrx{G}_s \vect{w}_s(\tau) d\tau,
\end{equation}
can also be shown to be zero-mean Gaussian using formulas \eqref{mean}
and \eqref{var}, such that $\vect{w}_{s_k} \sim
\mathcal{N}(0,\mtrx{Q}_{s_k})$. Due to the structure of
$\mtrx{F}_{s_k}$, we can also significantly simplify the covariance matrix:
\begin{align}
\mtrx{Q}_{s_k} &= \int^T_0 e^{\mtrx{F} (T-\tau)} \mtrx{G} \mtrx{Q} \mtrx{G}^\top e^{\mtrx{F}^\top (T-\tau)} d\tau \nonumber \\
&= \int^T_0
\left[\begin{array}{ccc}
\mtrx{I}&\mtrx{I}(T-\tau)&\mtrx{0}\\
\mtrx{0}&\mtrx{I}&\mtrx{I}(T-\tau)\\
\mtrx{0}&\mtrx{0}&\mtrx{I} \end{array} \right]
\left[\begin{array}{c}
\mtrx{0}\\
\mtrx{I}\\
\mtrx{0} \end{array} \right]
\mtrx{Q}_s
\left[\begin{array}{c}
\mtrx{0}\\
\mtrx{I}\\
\mtrx{0} \end{array} \right]^\top
\left[\begin{array}{ccc}
\mtrx{I}&\mtrx{I}(T-\tau)&\mtrx{0}\\
\mtrx{0}&\mtrx{I}&\mtrx{I}(T-\tau)\\
\mtrx{0}&\mtrx{0}&\mtrx{I} \end{array} \right]
 d\tau \nonumber \\
&= \left[\begin{array}{ccc}
\frac{1}{3}T^3&\frac{1}{2}T^2&0 \\
\frac{1}{2}T^2&T             &0 \\
0             &0             &0 \end{array} \right] \mtrx{Q}_s,
\end{align}
which, as expected, is singular, beacuse the velocity term is an exact
derivative of the acceleration term with no additive noise.


\subsection{Process Prediction}
\label{sec:proc_pred}

The complete state process prediction is found by substituting the
discrete-time linearized or linear vehicle process model (\eqref{disc_v} or \eqref{disc_s} respectively) into the
discrete-time linearized Kalman process prediction
equation \eqref{ekfpred1lin},
%
\begin{align}
\vect{\mu}_{k+1|k} &= \mtrx{F}_k \vect{\mu}_{k|k} + \mtrx{B}_{v_k} \vect{u}_k 
\label{nonlin_procpred}\\
\mtrx{\Sigma}_{k+1|k} &= \mtrx{F}_k \mtrx{\Sigma}_{k|k} \mtrx{F}_k^\top + \mtrx{Q}_k
\label{nonlin_procpredP}
\end{align}
where $\vect{\mu}$ and $\mtrx{\Sigma}$ are the mean and covariance,
respectively, of the estimate of the state $\vect{x}$ and
$\mtrx{Q}_k$ is defined above.





\subsection{Measurement Models}
\label{sec:meas_model}

To be updated.

\begin{itemize}
\item accelXYZ -- this is the only measurement used by the filter, but its in body
  frame, must be rotated into local-level frame to inform
  $\ddot{x}\ddot{y}\ddot{z}$ states
\item gyroXYZ -- ignore this and filter only RPH
\item magXYZ -- ignore this as well
\item head, pitch, roll -- processpressing to smooth RPH and then use ``as is''
  in order to transform linear accelerations from body frame to local-level
  frame
\item USBL -- provides ground truth for position $xyz$ at much lower update rate
  than accelXYZ data
\end{itemize}

%% Measurements from additional navigation sensors are
%% processed asynchronously using standard observation models
%% \cite{reustice-phdthesis}. On the vehicle, the depth sensor provides
%% observations of the vehicle's depth in the local-level coordinate
%% frame. The velocity sensor, a Doppler velocity log, provides
%% observations of the seafloor-relative velocity of the vehicle in the
%% sensor coordinate frame. The OCTANS sensor provides observations of
%% the vehicle's local-level attitude and body-frame angular rates. We
%% assume zero-mean, Gaussian noise for all of these sensor measurements
%% with standard deviations commensurate with the specifications of the
%% instrument manufacturers.

